Two-Sided Matching Markets: Impossibility Results on Existence of Efficient and Envy Free Solutions

The Hylland-Zeckhauser gave a classic pricing-based mechanism (HZ) for a one-sided matching market; it yields allocations satisfying Pareto optimality and envy-freeness (Hylland and Zeckhauser, 1979), and the mechanism is incentive compatible in the large (He et al., 2018). They also studied the exchange extension of HZ and gave an example showing that it may not even admit an equilibrium. In this paper, we consider two models of two sided matching markets: when utility functions are symmetric and when they are non-symmetric. We ask if these models always admit allocations satisfying the two basic properties of Pareto efficiency and envy freeness. Our results are negative. A corollary of the former result is a negative result for non-bipartite matching markets as well.

==> related.tex <==


\subsection{Related Results}
\label{sec.related}


The first comprehensive study of the computational complexity of the HZ scheme was undertaken in \cite{VY}. On the positive side, they gave a combinatorial, strongly polynomial time algorithm for the dichotomous case, i.e., 0/1 utilities, and extended it to the case that the utilities of each agent come from a set of cardinality two, i.e., a bivalued set; however, the set is allowed to be different for different agents. Clearly, for this case, the equilibrium is expressible using rational numbers. In contrast, they gave an example in which the utilities of agents come from a set of cardinality four for which an HZ equilibrium is not be expressible using rational numbers. Most importantly, they showed that the problem of approximately computing an equilibrium is in PPAD, though they left open the problem of showing PPAD-hardness. In particular, they stated that the problem should be PPAD-hard even if utilities of agents come from a set of cardinality three and that there should be an irrational example for this case as well. \cite{HZ-hardness} established PPAD-hardness, even if utilities of agents come from a set of cardinality four. 

This development opened up the question of finding tractable models of matching markets under cardinal utilities. \cite{HV-NBMM} addressed this question as detailed in the Introduction. In particular, they gave very general models of matching markets for which the resulting convex program has linear constraints thereby ensuring zero duality gap and polynomial time solvability. However, as is well known, polynomial time solvability is often just the beginning of the process of obtaining an ``industrial grade''  implementation. Towards this end, \cite{HV-NBMM} gave very fast implementations, using available solvers, and left the open problem of giving implementations with proven running times. The implementation given in \cite{HV-NBMM} can solve very large instances, with $n = 2000$, in one hour even for a two-sided matching market.


To deal with the fact that the Arrow-Debreu extension of HZ does not always admit an equilibrium, \cite{Echenique2019constrained} defined the notion of an $\alpha$-slack Walrasian equilibrium. This is a hybrid between the Fisher and Arrow-Debreu settings. Agents have initial endowments of goods and for a fixed $\alpha \in (0, 1]$, the budget of each agent, for given prices of goods, is $\alpha + (1 - \alpha) \cdot m$, where $m$ is the value for her initial endowment; the agent spends this budget to obtain an optimal bundle of goods. Via a non-trivial proof, they showed that for $\alpha > 0$, an $\alpha$-slack Walrasian equilibrium always exists.

\cite{Garg-ADHZ} gave the notion of an $\epsilon$-approximate Arrow-Debreu HZ equilibrium and using the result stated above on $\alpha$-slack Walrasian equilibrium, they showed that such an equilibrium always exists. They also gave a polynomial time algorithm for computing such an equilibrium for the dichotomous and bivalued utility functions.

An interesting recent paper \cite{Abebe-MM-Truthful} defines the notion of a random partial improvement mechanism for a one-sided matching market. This mechanism truthfully elicits the cardinal preferences of the agents and outputs a distribution over matchings that approximates every agent’s utility in the Nash bargaining solution.

In recent years, several researchers have proposed Hylland-Zeckhauser-type mechanisms for a number of applications, e.g., see \cite{Budish2011combinatorial, He2018pseudo, Le2017competitive, Mclennan2018efficient}. The basic scheme has also been generalized in several different directions, including two-sided matching markets, adding quantitative constraints, and to the setting in which agents have initial endowments of goods instead of money, see  \cite{Echenique2019constrained, Echenique2019fairness}.


